You Cannot Pick a Provider From the Price List: Market-Aware Routing for Open-Weight LLM Inference

Existing LLM routers choose among models using static per-model costs. We show that open-weight inference markets introduce a second, largely ignored decision axis: after choosing a model, a client must still choose which provider serves it. Measuring live endpoints across [nummodels] open models, competing providers, multiple task types, and three measurement waves, we find that provider choice cannot be inferred from the price list. The same model can vary sharply in quality, latency, availability, and price across providers; higher-priced providers are consistently faster, but price does not reliably predict quality or availability; and provider feasibility is task-selective, with one deployment nearly normal on knowledge tasks but catastrophically degraded on multi-step reasoning. We formulate same-model provider selection as a price-taker market-aware routing problem. A simple measured-map policy routes to the cheapest provider that is both quality-equivalent and healthy, yielding matched-quality savings while avoiding degraded endpoints. Because the map drifts, we introduce FACET, an online provider router that certifies per-(provider x task) feasibility facets and fails safe to an anchor before serving uncertified arms. Across relaxed deployment assumptions, FACET tolerates imperfect task assignment and sparse feedback, while systematic evaluator bias exposes a quality-signal trust boundary that can be mitigated with ground-truth probes or audits. Live provider runs further confirm that certification can move real traffic from a premium anchor to a substantially cheaper certified endpoint. Our results suggest that market-aware LLM routing must measure not only which model to use, but also who serves it.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table/baselines_table.tex <==
\begin{tabular}{lcccc}
\toprule
Policy & Mean acc.\ & Rel.\ cost$^\ast$ & Below-floor & Mean avail.\ \\
\midrule
Single-best (quality-first) & 95\% & 1.66$\times$ & 0\% & 96\% \\
Premium (most expensive) & 92\% & 3.67$\times$ & 17\% & 95\% \\
Random & 92\% & 2.19$\times$ & 22\% & 98\% \\
Cheapest (price-blind) & 91\% & 1.00$\times$ & 28\% & 97\% \\
\textbf{Ours} & 94\% & 1.57$\times$ & 0\% & 99\% \\
\bottomrule
\end{tabular}

==> table/bench_table.tex <==

\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}lrcccc@{}}
\toprule
Model & $|P|$ & Acc.\ range & Cheapest (acc @ \$/1M) & Worst (acc @ \$/1M) & Sep.\ \\
\midrule
\multicolumn{6}{l}{\emph{GSM8K}} \\
DeepSeek-v3.1 & 8 & 94--96\% & DeepInfra (96\% @ \$0.60) & Mara (94\% @ \$1.15) & --- \\
Gemma-3-27B & 4 & 93--95\% & DeepInfra (94\% @ \$0.12) & Parasail (93\% @ \$0.27) & --- \\
Llama-3.1-8B & 5 & 76--85\% & DeepInfra (79\% @ \$0.03) & Novita (76\% @ \$0.03) & --- \\
Llama-3.3-70B & 11 & 56--96\% & DeepInfra (96\% @ \$0.21) & Cloudflare (56\% @ \$1.27) & $\checkmark$ \\
Llama-4-Maverick & 5 & 95--97\% & DigitalOcean (96\% @ \$0.45) & Google (95\% @ \$0.75) & --- \\
Mistral-Small-24B & 2 & 96--97\% & Venice (97\% @ \$0.17) & Parasail (96\% @ \$0.19) & --- \\
\midrule
\multicolumn{6}{l}{\emph{MMLU}} \\
DeepSeek-v3.1 & 6 & 85--91\% & DeepInfra (85\% @ \$0.60) & CoreWeave (85\% @ \$1.10) & --- \\
Gemma-3-27B & 4 & 78--80\% & DeepInfra (78\% @ \$0.12) & Parasail (78\% @ \$0.27) & --- \\
Llama-3.1-8B & 5 & 64--68\% & DeepInfra (64\% @ \$0.03) & DeepInfra (64\% @ \$0.03) & --- \\
Llama-3.3-70B & 11 & 78--84\% & DeepInfra (81\% @ \$0.21) & Cloudflare (78\% @ \$1.27) & --- \\
Llama-4-Maverick & 5 & 77--84\% & DigitalOcean (83\% @ \$0.45) & Google (77\% @ \$0.75) & --- \\
Mistral-Small-24B & 2 & 80--81\% & DeepInfra (81\% @ \$0.14) & Venice (80\% @ \$0.17) & --- \\
\midrule
\multicolumn{6}{l}{\emph{HUMANEVAL}} \\
DeepSeek-v3.1 & 5 & 91--92\% & AtlasCloud (91\% @ \$0.62) & SiliconFlow (91\% @ \$0.64) & --- \\
Gemma-3-27B & 2 & 84--85\% & Nebius (85\% @ \$0.20) & Parasail (84\% @ \$0.27) & --- \\
Llama-3.1-8B & 5 & 59--70\% & DeepInfra (59\% @ \$0.03) & DeepInfra (59\% @ \$0.03) & --- \\
Llama-3.3-70B & 9 & 63--84\% & DeepInfra (84\% @ \$0.21) & Cloudflare (63\% @ \$1.27) & $\checkmark$ \\
Llama-4-Maverick & 4 & 85--89\% & DeepInfra (89\% @ \$0.50) & Google (85\% @ \$0.75) & --- \\
\bottomrule
\end{tabular}
\end{adjustbox}

==> table/context_table.tex <==
\begin{tabular}{lc}
\toprule
Certification granularity & Task-selective-mine serve rate \\
\midrule
Context-blind (one label per provider) & $6.7\%$ \\
\textbf{Per-(provider$\times$task) facet} & $\mathbf{0.0\%}$ \\
\bottomrule
\end{tabular}


==> table/facet_table.tex <==
\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{2}{c}{S1} & \multicolumn{2}{c}{S2} & \multicolumn{2}{c}{S3} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
Policy & cat\% & \$ & cat\% & \$ & cat\% & \$ \\
\midrule
\textsc{facet} core (optimistic election) & 0.4 & 1244 & 0.5 & 1179 & 0.9 & 1161 \\
\;$\hookrightarrow$ $-$anchor (ablation) & 0.4 & 1244 & 0.5 & 1179 & 0.9 & 1161 \\
\textbf{FACET (fail-safe)} & 0.0 & 1484 & 0.6 & 1444 & 1.3 & 1332 \\
\bottomrule
\end{tabular}

==> table/oos_table.tex <==
\begin{tabular}{lccc@{\hskip 14pt}ccc}
\toprule
& \multicolumn{3}{c}{In-sample (map on its own wave)} & \multicolumn{3}{c}{\emph{Out-of-sample} (aged map on later wave)} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Policy & Acc & Below-fl & q-reg & Acc & Below-fl & q-reg \\
\midrule
Single-best & 87\% & 0\% & 0.0 & 87\% & 0\% & 0.0 \\
\textbf{Router (ours)} & 85\% & 0\% & 0.0 & 86\% & 11\% & 0.0 \\
Cheapest & 84\% & 22\% & 0.1 & 85\% & 22\% & 0.1 \\
Premium & 79\% & 44\% & 4.3 & 80\% & 33\% & 4.0 \\
\bottomrule
\end{tabular}

==> table/results_table.tex <==
% \begin{tabular}{llrccccr}
% \toprule
% Model & Task & $|P|$ & Acc.\ range & Price$\times$ & Lat.$\times$ & Route price & Save \\
% \midrule
% deepseek-chat-v3.1 & classification & 7 & 100\%--100\% & 2.3 & 68 & \$0.500 & 57\% \\
%  & extraction & 6 & 93\%--100\% & 1.8 & 34 & \$0.625 & 46\% \\
%  & math & 7 & 100\%--100\% & 2.3 & 24 & \$0.625 & 46\% \\
% gemma-3-27b-it & classification & 5 & 100\%--100\% & 2.5 & 4 & \$0.120 & 61\% \\
%  & extraction & 5 & 100\%--100\% & 2.5 & 8 & \$0.120 & 61\% \\
%  & math & 4 & 53\%--72\%\,$\dagger$ & 1.9 & 3 & \$0.305 & 0\% \\
% llama-3.1-8b-instruct & classification & 5 & 100\%--100\% & 8.8 & 8 & \$0.025 & 89\% \\
%  & extraction & 5 & 80\%--93\%\,$\dagger$ & 8.8 & 10 & \$0.035 & 84\% \\
%  & math & 5 & 56\%--85\%\,$\dagger$ & 8.8 & 13 & \$0.220 & 0\% \\
% llama-3.3-70b-instruct & classification & 9 & 100\%--100\% & 4.8 & 25 & \$0.265 & 79\% \\
%  & extraction & 10 & 93\%--100\% & 5.0 & 6 & \$0.210 & 80\% \\
%  & math & 11 & 40\%--75\%\,$\dagger$ & 6.1 & 56 & \$0.265 & 79\% \\
% llama-4-maverick & classification & 4 & 100\%--100\% & 2.0 & 3 & \$0.375 & 50\% \\
%  & extraction & 4 & 93\%--93\% & 2.0 & 4 & \$0.375 & 50\% \\
%  & math & 4 & 80\%--85\% & 2.0 & 2 & \$0.375 & 50\% \\
% mistral-small-3.2-\\24b-instruct & classification & 4 & 100\%--100\% & 1.5 & 2 & \$0.172 & 14\% \\
%  & extraction & 4 & 93\%--100\%\,$\dagger$ & 1.5 & 3 & \$0.200 & 0\% \\
%  & math & 4 & 100\%--100\% & 1.5 & 4 & \$0.138 & 31\% \\
% \bottomrule
% \end{tabular}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llrccccr}
\toprule
&&&
\multicolumn{3}{c}{\textbf{Provider heterogeneity}}
&
\multicolumn{2}{c}{\textbf{Routing outcome}} \\
\cmidrule(lr){4-6}
\cmidrule(lr){7-8}
Model & Task & $|P|$ & Acc.\ range & Price$\times$ & Lat.$\times$
& Route price & Save \\
\midrule

deepseek-chat-v3.1
& classification & 7 & 100\%--100\% & 2.3 & \textbf{68} & \$0.500 & 57\% \\
& extraction & 6 & 93\%--100\% & 1.8 & 34 & \$0.625 & 46\% \\
& math & 7 & 100\%--100\% & 2.3 & 24 & \$0.625 & 46\% \\

\addlinespace[2pt]

gemma-3-27b-it
& classification & 5 & 100\%--100\% & 2.5 & 4 & \$0.120 & 61\% \\
& extraction & 5 & 100\%--100\% & 2.5 & 8 & \$0.120 & 61\% \\
& math & 4 & 53\%--72\%\,$\dagger$ & 1.9 & 3 & \$0.305 & 0\% \\

\addlinespace[2pt]

llama-3.1-8b-instruct
& classification & 5 & 100\%--100\% & 8.8 & 8 & \$0.025 & \textbf{89\%} \\
& extraction & 5 & 80\%--93\%\,$\dagger$ & 8.8 & 10 & \$0.035 & \textbf{84\%} \\
& math & 5 & \textbf{56\%--85\%}\,$\dagger$ & 8.8 & 13 & \$0.220 & 0\% \\

\addlinespace[2pt]

llama-3.3-70b-instruct
& classification & 9 & 100\%--100\% & 4.8 & 25 & \$0.265 & 79\% \\
& extraction & 10 & 93\%--100\% & 5.0 & 6 & \$0.210 & \textbf{80\%} \\
& math & 11 & \textbf{40\%--75\%}\,$\dagger$ & 6.1 & \textbf{56} & \$0.265 & 79\% \\

\addlinespace[2pt]

llama-4-maverick
& classification & 4 & 100\%--100\% & 2.0 & 3 & \$0.375 & 50\% \\
& extraction & 4 & 93\%--93\% & 2.0 & 4 & \$0.375 & 50\% \\
& math & 4 & 80\%--85\% & 2.0 & 2 & \$0.375 & 50\% \\

\addlinespace[2pt]

mistral-small-3.2-24b-instruct
& classification & 4 & 100\%--100\% & 1.5 & 2 & \$0.172 & 14\% \\
& extraction & 4 & 93\%--100\%\,$\dagger$ & 1.5 & 3 & \$0.200 & 0\% \\
& math & 4 & 100\%--100\% & 1.5 & 4 & \$0.138 & 31\% \\

\bottomrule
\end{tabular}%
}

==> table/scope_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
 & Cost prem.\ & \multicolumn{2}{c}{Below-floor rate} & \multicolumn{2}{c}{Quality-regret} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Policy & vs oracle & median & \emph{worst} & median & \emph{worst} \\
\midrule
Static-argmin & -6\% & 33.0\% & 33.0\% & 49.50 & 49.50 \\
Cost-Thompson & +4\% & 6.5\% & 47.6\% & 9.08 & 20.45 \\
SW-UCB & +13\% & 2.4\% & 56.6\% & 3.33 & 6.26 \\
M-UCB (change-detect) & +14\% & 2.5\% & 53.2\% & 3.71 & 6.17 \\
\textbf{\textsc{facet}} core & +59\% & 1.3\% & 42.6\% & 1.78 & 4.41 \\
\bottomrule
\end{tabular}
